DoCRL: Double Critic Deep Reinforcement Learning for Mapless Navigation of a Hybrid Aerial Underwater Vehicle with Medium Transition

Deep Reinforcement Learning (Deep-RL) techniques for motion control have been continuously used to deal with decision-making problems for a wide variety of robots. Previous works showed that Deep-RL can be applied to perform mapless navigation, including the medium transition of Hybrid Unmanned Aerial Underwater Vehicles (HUAUVs). These are robots that can operate in both air and water media, with future potential for rescue tasks in robotics. This paper presents new approaches based on the state-of-the-art Double Critic Actor-Critic algorithms to address the navigation and medium transition problems for a HUAUV. We show that double-critic Deep-RL with Recurrent Neural Networks using range data and relative localization solely improves the navigation performance of HUAUVs. Our DoCRL approaches achieved better navigation and transitioning capability, outperforming previous approaches.

==> whatever/sections/0_0_abstract.tex <==
\begin{abstract}
%ICRA
% Since the application of Deep Q-Learning to the continuous action domain in Atari-like games, Deep Reinforcement Learning (Deep-RL) techniques for motion control have been qualitatively enhanced. Nowadays, modern Deep-RL can be successfully applied to solve a wide range of complex decision-making tasks for many types of vehicles. 
% Based on this context, in this paper, we propose the use of Deep-RL to perform autonomous mapless navigation for Hybrid Unmanned Aerial Underwater Vehicles (HUAUVs), robots that can operate in both, air or water media. We developed two approaches, one deterministic and the other stochastic. Our system uses the relative localization of the vehicle and simple sparse range data to train the network. We compared our approaches with an adapted version of the BUG2 algorithm for mapless navigation of aerial vehicles. Based on experimental results, we can conclude that Deep-RL-based approaches can be successfully used to perform mapless navigation and obstacle avoidance for HUAUVs. Our vehicle accomplished the navigation in two scenarios, being capable to achieve the desired target through both environments, and even outperforming the behavior-based algorithm on the obstacle-avoidance capability.
Deep Reinforcement Learning (Deep-RL) techniques for motion control have been continuously used to deal with decision-making problems for a wide variety of robots. Previous works showed that Deep-RL can be applied to perform mapless navigation, including the medium transition of Hybrid Unmanned Aerial Underwater Vehicles (HUAUVs). These are robots that can operate in both air and water media, with future potential for rescue tasks in robotics. This paper presents new approaches based on the state-of-the-art Double Critic Actor-Critic algorithms to address the navigation and medium transition problems for a HUAUV. We show that double-critic Deep-RL with Recurrent Neural Networks using range data and relative localization solely improves the navigation performance of HUAUVs. Our DoCRL approaches achieved better navigation and transitioning capability, outperforming previous approaches. 
\end{abstract}
%\vspace{-1mm}

% \begin{IEEEkeywords}
% Deep Reinforcement Learning, Hybrid Unmanned Aerial Underwater Vehicle, Mapless Navigation
% \end{IEEEkeywords}


==> whatever/sections/0_1_supplementary_material.tex <==
\section*{Supplementary Material}\label{supplementary_material}

Video of the experiments available at: \texttt{\url{https://youtu.be/PqTDzsKjA9c}}. 
Released code at: \texttt{\url{https://github.com/ricardoGrando/DoCRL}}. 



==> whatever/sections/1_introduction.tex <==
\section{Introduction}
\label{introduction}

% In the last few years, Deep Reinforcement Learning (Deep-RL) has been increasingly employed in a wide range of fields. Promising results have been achieved in tasks involving control and discrete systems \cite{mnih2013playing}, \cite{schaul2015prioritized}, and continuous systems \cite{lillicrap2015continuous}. In Robotics, Deep-RL was first applied to handling tasks in stable and observable environments \cite{gu2016continuous}. For mobile robots, however, there is a significant increase in complexity due to interactions with barriers in the physical workspace. In this context, Deep-RL approaches typically concentrate on discretizing the problem to solve it \cite{zhu2017target}. 

Several studies about Hybrid Unmanned Aerial Underwater Vehicles (HUAUVs) have been conducted recently \cite{drews2014hybrid, neto2015attitude, da2018comparative, maia2017design, lu2019multimodal, mercado2019aerial,horn20,aoki2021}. These vehicles provide an interesting range of possible applications due to the capability to act in two different environments, including inspection and mapping of partly submerged areas in industrial facilities, search and rescue and other military-related applications. However, the state-of-the-art is yet focused on the vehicle design and structure, where even fewer studies around autonomous navigation have been conducted \cite{bedin2021deep}. The ability to perform tasks in both environments and successfully transit between them imposes additional challenges that must be addressed to make this mobile vehicle autonomously feasible. 

\begin{figure}[tbp!]
    \vspace{-2mm}
    \centering
    \includegraphics[width=\linewidth]{img/scheme.png}
    \caption{DoCRL architecture.}
    \label{fig:system_def}
    \vspace{-4mm}
\end{figure}

Approaches based on Deep Reinforcement Learning (Deep-RL) techniques have been enhanced to address navigation-related tasks for a range of mobile vehicles, including ground mobile robots \cite{ota2020efficient}, aerial robots \cite{tong2021uav,grando2022double} and underwater robots \cite{carlucho2018}. These approaches based on single critic actor-critic techniques with multi-layer network structures have achieved interesting results in performing mapless navigation, obstacle avoidance and media transitioning even for HUAUVs \cite{bedin2021deep}. However, the challenges faced by this kind of vehicle make these approaches limited, not being capable of escalating to more complex scenarios for a rescue navigation task, for example.

% Falar da motivação:
% Como o artigo melhora as abordagens anteriores?

In this work, we explore the use of Deep-RL in the context of HUAUVs to perform navigation-related tasks that can simulate through environmental rescue tasks in robotics. We present two enhanced approaches based on state-of-the-art Deep-RL for the continuous state:  (1) a deterministic based on Twin Delayed Deep Deterministic Policy Gradient (TD3) \cite{fujimoto2018addressing}; and
 (2) a stochastic based on Soft Actor-Critic (SAC) \cite{haarnoja2018soft}. We show that we are capable of training agents with a consistently better capability than state-of-the-art, performing with more stability the mapless navigation, obstacle avoidance and medium transition. We perform a two-fold way evaluation with air-to-water and water-to-air navigation. We compare our DoCRL approaches with single critic-based approaches used to perform mapless navigation and with an adapted version of a traditional Behavior-Based Algorithm (BBA) \cite{marino2016minimalistic} used in aerial vehicles. Our proposed double critic formulation can be seen in Fig. \ref{fig:system_def}.
 
 %, emulated in the Gazebo simulator. 

% In this work, we focus on demonstrating the effectiveness of Deep-RL on the mapless navigation of HUAUVs. More specifically, we tackled the task of goal-oriented navigation with a medium transition in a two-fold way for the HUAUV presented in \cite{drews2014hybrid}. We proposed two approaches: 
% 1) A deterministic based on Deep Deterministic Policy Gradient (DDPG);
% 2) A stochastic based on Soft Actor-Critic (SAC).
% We train and test in two different scenarios with both approaches, then compare the results with a version of the BUG2 algorithm inspired in the work of Marino et al. \cite{marino2016minimalistic} for aerial vehicles. Our system definition can be seen in Fig. \ref{fig:system_def}.%, emulated in the Gazebo simulator. 

% \begin{figure}[tbp!]
%     \centering
%     \includegraphics[width=\linewidth]{img/system_full_new_3.png}
%     \caption{Our HUAUV performing in the third scenario (left) and the deterministic and stochastic DoCRL structures with inputs and outputs (right).}
%     \label{fig:system_def}
%     \vspace{-6mm}
% \end{figure}



%The main contributions of this work are listed as follows:

This work contains the following main contributions:

\begin{itemize}

\item We propose two approaches based on state-of-the-art actor-critic double critic Deep-RL algorithms that can successfully perform goal-oriented mapless navigation for HUAUVs, using only range data readings and the vehicles' relative localization data.

\item We show that a Long Short Term Memory (LSTM) architecture achieves better overall performance than the state-of-the-art Multi-Layer Perceptron (MLP) architecture.%, commonly used for mobile robots \cite{tai2017virtual, singh2018mobile, bedin2021deep}.

% \item We present a simulated hybrid vehicle with more realistic sensing, coupled with a real-world described LIDAR for aerial sensing and underwater Forward Looking Sonar (FLS) for underwater sensing. We provide a package with our real-world described HUAUV, completely built on Robot Operating System (ROS) and Gazebo simulator.

\item We show that our robot presents a robust capacity to navigate in scenarios that can simulate through environmental (air-water) rescue tasks in robotics. The robot also performs the medium transition, capable of arriving at the desired target and avoiding collisions.

% \item Most importantly, we show that our methodology and the scenario setup can be escalated for tasks of rescue in robotics for this specific kind of hybrid vehicle.

\end{itemize}

This work has the following structure: the related works are discussed in the following section (Sec. \ref{related_works}). Following it, we present our methodology in Sec. \ref{methodology}. The results are presented in Sec. \ref{results} and discussed in Sec. \ref{discussion}. Finally, we discuss our contributions and present future works in Sec. \ref{conclusion}.


==> whatever/sections/2_related_works.tex <==
\section{Related Work}
\label{related_works}

The HUAUV literature is still mostly concerned with mechanical design and modelling \cite{drews2014hybrid, neto2015attitude, da2018comparative, maia2017design, lu2019multimodal, mercado2019aerial, horn20}. Autonomous navigation-related problems are still barely addressed for this kind of vehicle \cite{bedin2021deep}. The HUAUV used in this paper \cite{bedin2021deep} was created based on Drews-Jr \emph{et al.} \cite{drews2014hybrid} model, which Neto \emph{et al.} \cite{neto2015attitude} has largely expanded.

%iruthayanathan2016performance,

Several Deep-RL works in robotics have previously been carried out for the mapless navigation problem, demonstrating how efficiently we may solve the problem utilizing learning techniques% %\cite{kober2013reinforcement,kormushev2013reinforcement,
~\cite{tobin2017domain}. For a mapless motion planner of a ground robot, Tai \emph{et al.} \cite{tai2017virtual} employed 10-dimensional range findings and the relative distance of the vehicle to a target as inputs and continuous steering signals as outputs. According to the results, a mapless motion planner based on the DDPG algorithm may be effectively taught and utilized to navigate to a target. Recently, deep-RL methods have also been successfully used in robotics by %Zhu \emph{et al.} \cite{zhu2017target}, Chen \emph{et al.} \cite{chen2017socially}, 
Ota \emph{et al.} \cite{ota2020efficient}, de Jesus \emph{et al.}. \cite{jesus2019deep,jesus2021soft}, and others to accomplish mapless navigation-related tasks for terrestrial mobile robots. 

% He \emph{et al.} \cite{he2021lane} proposes a lane following method using an improved DDPG algorithm based on the double critic networks and priority experience replay mechanism to perform autonomous drive navigation. He \emph{et al.} Experiments show that the algorithm can achieve excellent following results under various road conditions.

Kelchtermans and Tuytelaars \cite{kelchtermans2017hard} used a LSTM to perform autonomous navigation in a UAV. The room crossing task performed by Kelchtermans and Tuytelaars approach demonstrated through simulation how memory can help Deep Neural Networks (DNN) in navigation control. Tong \emph{et al.} \cite{tong2021uav} proposed a DRL-based method using a LSTM to navigate a UAV in high dynamic environments, with numerous obstacles moving fast. Their approach achieved superiority in terms of convergence and effectiveness compared with the state-of-the-art DRL methods. 
Singh and Thongam \cite{singh2018mobile} employed a Multi-Layer Perceptron (MLP) to perform terrestrial mobile robot navigation in dynamic environments. Their method is used to choose a collision-free segment and controls the robot's speed for each motion. They demonstrated that the method is efficient and gives a near-optimal path reaching the target position of the mobile robot.

% repetido, ja falou do tai antes
% When applied to mobile robots, Tai \emph{et al.} \cite{tai2017virtual} used 10-dimensional range findings and a goal location as inputs and continuous steering directives as outputs for a 2D mapless motion planner. They determined that using the DDPG method with a MLP with three hidden layers will effectively train a 2D mapless motion planner. Furthermore, the task of accomplishing the objective of reaching a predetermined target was effectively performed. 

When it comes to problems involving mapless navigation for Unmanned Aerial Vehicles, the effectiveness of Deep-RL is somewhat limited (UAVs) \cite{grando2020visual}. Rodriguez \emph{et al.} \cite{rodriguez2018deep} employed a DDPG-based strategy to solve the problem of landing on a moving platform. It employed Deep-RL in conjunction with the RotorS framework \cite{furrer2016rotors} to simulate UAVs in the Gazebo simulator. Sampedro \emph{et al.} \cite{sampedro2019fully} proposed a DDPG-based strategy for the Search and Rescue mission in interior situations, utilizing visual data from a real and simulated UAV. Kang \emph{et al.} \cite{kang2019generalization} also used visual information, although he focused on the subject of collision avoidance. In a go-to-target task, Barros \emph{et al.} \cite{2020arXiv201002293M} applied a SAC-based method to low-level control of a UAV. Grando \emph{et al.} \cite{grando2020deep} utilized approaches based on the DDPG and SAC algorithms on Gazebo for 2D UAV navigation. Recently, double critic-based Deep-RL approaches have been developed for UAVs, presenting better results \cite{grando2022double}.

% nao é um trabalho relacionado, mas uma ferramenta que utilizamos
% Cerqueira \emph{et al.} \cite{cerqueira2017novel} proposed a system to work with simulated AUV. Their approach can simulate two main types of acoustic devices: mechanical scanning imaging sonars and forward-looking sonars. Cerqueira \emph{et al.} method generates visually realistic sonar images when compared with real-world sonar images of the same scenes, and the evaluation demonstrated that the proposed system can operate close to or faster than real-world devices.


%Our previous deterministic approach 3DNDRL-D \cite{bedin2021deep} was used for comparison.
%This stochastic approach is an extension of our previous stochastic approach 3DNDRL-S \cite{bedin2021deep}

Two works have recently tackled the navigation problem with the medium transition of HUAUVs \cite{pinheiro2021trajectory}, \cite{bedin2021deep}. Pinheiro \emph{et al.} \cite{pinheiro2021trajectory} focused on smoothing the medium transition problem in a simulated model on MATLAB. Grando \emph{et al.} \cite{bedin2021deep} developed Deep-RL approaches following single critic structure and a MLP architecture. These two works were developed using generic distance sensing information for aerial and underwater navigation. In contrast, more sophisticated sensing with a real-world simulated LIDAR and sonar is adopted in the present work.

Our work differs from the previously discussed works by only using the vehicle's relative localization data and not its explicit localization data. We also present Deep-RL approaches based on double critic techniques instead of single critic, with RNN structures instead of MLP, traditionally used for mapless navigation of mobile robots. We compare our DoCRL approaches with state-of-the-art Deep-RL approaches and with a behavior-based algorithm \cite{marino2016minimalistic} adapted for hybrid vehicles to show that our methodology improves the overall capability to perform autonomous navigation.


==> whatever/sections/3_methodology.tex <==
\section{Methodology}
\label{methodology}

In this section, we discuss our Deep-RL approaches. We detail the network structure for both deterministic and stochastic agents. We also present the proposed reward function for the task that the vehicle must accomplish autonomously.

%%DREWS\subsection{Deep Reinforcement Learning}% Reescrito por Alisson

%Deep reinforcement learning makes use of reinforcement learning and neural networks.
%With this two techOne of the first algorithms to utilize Deep-RL was the deep Q-network (DQN) algorithm \cite{mnih2013playing} which managed to outperform humans in many games. Because DQN worked with discrete actions, its applications were restricted leading to the development of \cite{lillicrap2015continuous}, wich uses continuous action spaces.

%%%DREWS Deep reinforcement learning merges concepts of reinforcement learning, where we intend to teach an agent to provide the best action to maximize a reward function in a given state, with deep neural networks. One of the first algorithms to utilize Deep-RL was the deep Q-network (DQN) algorithm \cite{mnih2013playing} which managed to outperform humans in several games. Because DQN only works with discrete actions, its applications were restricted leading to the development of continuous action spaces \cite{lillicrap2015continuous}.
% aims to endow an agent with some capabilities by maximizing a reward function. By setting the agent's actions, the traditional deep Q-network (DQN) algorithm \cite{mnih2013playing} managed to outperform humans in many games. However, it only worked in discrete action spaces, being unable to handle complex observation spaces. Since many tasks in robot control have continuous action spaces and DQN was not designed for continuous domains, another algorithm must be used to deal with such a problem \cite{lillicrap2015continuous}.

\subsection{Double Critic Deep Reinforcement Learning Deterministic - DoCRL-D}% Reescrito por Alisson

Developing on the DQN \cite{mnih2013playing}, Deep Deterministic Policy Gradient (DDPG)~\cite{lillicrap2015continuous} employs an actor-network where output is a real value that represents a chosen action, and a second neural network to learn the target function providing stability and making it ideal for mobile robots~\cite{jesus2019deep}. While providing good results, DDPG still has its problems, like overestimating the Q-values leading to policy breaking. TD3 \cite{fujimoto2018addressing} uses DDPG as its backbone and improves it by adding some improvements, such as clipped double-Q learning with two neural networks as targets for the Bellman error loss functions, delayed policy updates, and Gaussian noise on the target action, raising its performance.    
%The DDPG architecture has been proposed as an extension to the DQN, and it became a founding block for Deep-RL applications of mobile robots in continuous observation spaces \cite{jesus2019deep}. It consists of an actor-critic approach that uses approximation functions to learn continuous space policies.
% Two neural networks are used, one for the actor and another for the critic. For each time step, the networks forecast the behavior for the current state and produce a temporal difference error signal. 
% The output of the critic-network is the Q-value for action, while the actor-network output is a real value that represents a chosen action.
Our deterministic approach is based on the TD3 technique. The pseudocode of DoCRL-D can be seen in Algorithm \ref{alg:docrl_d}.

\begin{algorithm}[!htb]
    \algsetup{linenosize=\tiny}
    \scriptsize
    \caption{Double Critic Deep Reinforcement Learning Deterministic - DoCRL-D}
    \label{alg:docrl_d}
    \begin{algorithmic}[1]
        \STATE Initialize params of critic networks $\theta_{1}$, $\theta_{2}$ , and actor network $\pi(\phi)$
        \STATE Initialize params of target networks $\phi^{\prime}\leftarrow\phi$, $\theta_{1}^{\prime}\leftarrow\theta_{1}$, $\theta_{2}^{\prime}\leftarrow\theta_{2}$
        \STATE Initialize replay buffer $\beta$
        \FOR{$ep = 1$ to $max\_eps$}
            \STATE reset environment state
            \FOR{$t = 0$ to $max\_steps$}
                \IF {$t < start\_steps$}
                    \STATE $a_{t} \leftarrow $ env.action\_space.sample() 
                %
                \ELSE
                    \STATE $a_{t}\leftarrow\pi_{\phi}(s)+\epsilon,\ \epsilon\sim \mathcal{N}(0,OU)$
                %
                \ENDIF
                
                \STATE $s_{t+1}$, $r_{t}$, $d_{t}$, \_ $\leftarrow$ env.step($a_{t}$)
                
                \STATE store the new transition $(s_{t}, a_{t}, r_{t}, s_{t+1}, d_{t})$ into $\beta$
                
                \IF{$t > start\_steps$}
                    \STATE Sample mini-batch of $N$ transitions $(s_{t}, a_{t}, r_{t},s_{t+1}, d_{t})$ from $\beta$
                    
                    \STATE $a'\leftarrow\pi_{\phi^{\prime}}(s^{\prime})+\epsilon,\ \epsilon\sim clip(\mathcal{N}(0,\tilde{\sigma}), -c,\ c)$ 
                    
                    \STATE Computes target: \\ $Q_{t} \leftarrow r+\gamma*\min_{i=1,2}Q_{\theta_i}(s', a')$
                    
                    % \STATE $\mathcal{L}oss_{\theta_i}=l_{MSE}(Q_{1}, Q_{t})+l_{MSE}(Q_{2},\ Q_{t})$
                    
                    \STATE Update double critics with one step gradient descent:\\
                   $\nabla_{\theta_i} \frac{1}{N} \sum_i(Q_t - Q_{\theta_{i}(s_{t},a_{t})})^2$  \qquad for i=1,2
                    
                    \IF {t \% policy\_freq == 0}
                        \STATE Update policy with one step gradient descent:\\             
                        $\nabla_{\phi}\frac{1}{N} \sum_i[\nabla_{a_{t}}Q_{\theta_{1}}(s_{t},a_{t})\vert _{a_{t}=\pi(\phi)}\nabla_{\phi}\pi_{\phi}(s_{t})]$
                        
                        Soft update for the target networks: \\
                        \STATE $\phi^{\prime}\leftarrow\tau\phi+(1-\tau)\phi^{\prime}$
                        \STATE $\theta_{i}^{\prime}\leftarrow\tau\theta_{i}+(1-\tau)\theta_{i}^{\prime}$ \qquad for i=1,2
                        
                        
                    \ENDIF
                \ENDIF
            \ENDFOR
        \ENDFOR
  \end{algorithmic}
\end{algorithm}

We train for a number max steps ($max\_steps$) in a number episodes ($max\_steps$). Our approach starts by exploring random actions while a minimum number of steps ($start\_steps$) has not been achieved yet.

We use an LSTM as actor-network and denote them by $\phi$ and its copy $\phi^{\prime}$ as actor target. The double critic as well, by $\theta_{1}$, $\theta_{2}$ for parameterization of two value networks and its copies $\theta_{1}^{\prime}$, $\theta_{2}^{\prime}$ as critic targets. The learning of both networks happens simultaneously, addressing approximation error, reducing the bias, and finding the highest Q-value. The actor target chooses the action $a^{\prime}$ based on the state $s^{\prime}$, and we add Ornstein-Uhlenbeck noise to it. The double critic targets take the tuple ($s^{\prime}$, $a^{\prime}$) and return two Q-values as output. The minimum of the two target Q-values is considered as the approximated value return. The loss is calculated with the Mean Squared Error of the approximate value from the target networks and the value from the critic networks. We use Adaptive Moment Estimation (Adam) to minimize the loss.

We delay by updating the policy network less frequently than the value network. It is updated taking into account a $policy\_freq$ factor that increases over time by the following rule:

\begin{equation*} policy\_freq=(int)\frac{1}{0.5- \frac{t}{max\_steps \times 3}}. \end{equation*}

\subsection{Double Critic Deep Reinforcement Learning Stochastic - DoCRL-S}% Reescrito por Alisson

A stochastic approach is also developed in this work. Our approach is based on the SAC algorithm~\cite{haarnoja2018soft}. This algorithm consists of a bias-stochastic actor-critic that combines off-policy updates with a stochastic actor-critic method to learn continuous action space policies. It uses neural networks as approximation functions to learn a policy and two Q-values functions similarly to TD3. However, SAC utilizes the current stochastic policy to act without noise, providing better stability and performance. It maximizes the reward and the policy's entropy, encouraging the agent to explore new states and improving training speed. We use the soft Bellman equation with neural networks as a function approximation to maximize the entropy. The pseudocode of DoCRL-S can be seen in Algorithm \ref{alg:docrl_s}.

\begin{algorithm}[!htb]
    \algsetup{linenosize=\tiny}
    \scriptsize
    \caption{Double Critic Deep Reinforcement Learning Stochastic - DoCRL-S}
    \label{alg:docrl_s}
    \begin{algorithmic}[1]
        \STATE Initialize critic networks $\theta_{1}$, $\theta_{2}$ , and actor network $\pi(\phi)$
        \STATE Initialize target networks $\phi^{\prime}\leftarrow\phi$, $\theta_{1}^{\prime}\leftarrow\theta_{1}$, $\theta_{2}^{\prime}\leftarrow\theta_{2}$
        \STATE Initialize replay buffer $\beta$
        \FOR{$ep = 1$ to $max\_eps$}
            \STATE reset environment state
            \FOR{$t = 0$ to $max\_steps$}
                \IF {$t < start\_steps$}
                    \STATE $a_{t}$ = env.action\_space.sample() 
                %
                \ELSE
                    \STATE $a_t\leftarrow\pi_{\phi}(\cdot|s)$
                %
                \ENDIF
                
                \STATE $s_{t+1}$, $r_{t}$, $d_{t}$, \_ env.step($a_{t}$)
                
                \STATE store the new transition $S$ $(s_{t}, a_{t}, r_{t}, s_{t+1}, d_{t})$ into $\beta$
                
                \IF{$t > start\_steps$}
                    \STATE Sample m-batch of $N$ transitions $(s_{t}, a_{t}, r_{t},s_{t+1}, d_{t})$ from $\beta$
                    
                    \STATE $double = ([min_{i=1,2}( Q_{\theta'_{i}}({s_{t}},{a_{t}}))-\alpha \log \pi ({a_{t}}|{s_{t}})])$
                    
                    \STATE $Q_t=r({s_{t}},{a_{t}})+\gamma(1-d_{t})*double$ 
                    
                    \STATE Update double critics with one step gradient descent:\\
                    $\nabla_{\theta_i} argmin_{\theta_{i}} \frac{1}{|N|} \sum(Q_t - Q_{\theta_{i}}(s_{t},a_{t}))^2$  \qquad for i=1,2
                    
                    \IF {t \% policy\_freq == 0}
                        
                        \STATE Update policy with one step gradient descent:\\
                        $ \nabla_{\phi} \frac{1}{|N|} \sum_{s_t \in \beta} ([min_{i=1,2}( Q_{\theta_{i}}({s_{t}},{a_{t_\phi}}))-\alpha \log \pi ({a_{t_\phi}}|{s_{t}})])$ \qquad for i=1,2
                        
                       
                        \STATE Soft update for the target networks:\\ $\theta_i^{\prime}\leftarrow\tau\theta_i+(1-\tau)\theta_i^{\prime}$ \qquad for i=1,2
                    \ENDIF
                \ENDIF
            \ENDFOR
        \ENDFOR
  \end{algorithmic}
\end{algorithm}

We train for a number max steps ($max\_steps$) in a number of episodes ($max\_steps$) as well. It explores random actions while a minimum number of steps ($start\_steps$) has not been achieved yet. A LSTM structure was used for the policy network $\phi$. After sampling a batch from the memory, we compute the targets for the Q-functions $Q_t({r_{t}},{s_{t+1}},{d_{t}})$, and update the Q-functions. We perform the delay by updating the policy less frequently than the value network, as performed with our DoCRL-D approach. It was updated taking into account the same $policy\_freq$ factor as the DoCRL-D. 

\subsection{Simulated Environments}% Reescrito por Alisson

Our experiments are conducted with the vehicle and on the second and more complex environment provided by Grando et al. \cite{bedin2021deep}. Based on the Gazebo simulator together with ROS, it makes the use of the framework RotorS \cite{furrer2016rotors}, which provides the means to simulate aerial vehicles with different command levels, such as angular rates, attitude, location control and the simulation of wind with an Ornstein-Uhlenbeck noise method. The underwater simulation is enabled by the UUV simulator \cite{manhaes2016uuv}, which allows the simulation of hydrostatic and hydrodynamic effects, as well as thrusters, sensors, and external perturbations. With this framework, the vehicle's underwater model was defined with parameters such as the volume,  additional mass, center of buoyancy, etc., as well as the characteristics of the underwater environment itself.

The environment simulate a walled water tank, with dimensions of 10$\times$10$\times$6 meters and a one-meter water column. It has four cylindrical columns representing drilling risers.
% The third environment simulates complex structures like those found in sea platforms and contains several elements, such as walls, half walls and pipes.

\subsubsection{HUAUV Description} % Reescrito por Ricardo

% \begin{figure}[tbp!]
%     %\vspace{-1mm}
%     \centering
%     \includegraphics[width=\linewidth]{img/sonar_v3.png}
%     \caption{Our HUAUV performing in the second scenario (left) and the Sonar sensing (right).}
%     \label{fig:sonar}
%     %\vspace{-6mm}
% \end{figure}

The vehicle used is based on the model presented by Drews-Jr \emph{et al.} \cite{drews2014hybrid}, Neto \emph{et al.} \cite{neto2015attitude} and \emph{et al.} \cite{horn2019study}. It was described using its actual mechanics settings, including the inertia, motor coefficients, mass, rotor velocity, and others. Its sensing was optimized for real-world LIDAR and Sonar. The described LIDAR is based on the UST 10LX model. It provides a 10 meters distance sensing with 270\degree range and 0.25\degree of resolution. It was simulated using the plugin ray of Gazebo. The simulated FLS sonar is based on the sonar simulation plugin developed by Cerqueira \emph{et al.}~\cite{cerqueira2017novel}. It has 20 meters of range, with a bin count of 1000 and a beam count of 256. The width and height angles of the beam were $90^0$ and $15^0$, respectively. 
% In the real world, the distance sensing can be yielded in the real world from its respective sensors, while the localization information can obtained from a combination of standard localization sensing of hybrid vehicles like Global Positioning System (GPS) and Ultra Short Baseline (USBL).

%\vspace{-2mm}
\subsubsection{Network Structure and Rewarding System} \label{secapproach}
%
% REESCREVER

% In this work, we aim 
% % that our described HUAUV manages 
% to navigate our described HUAUV autonomously from a starting point to a target point in a different environment without any environmental knowledge, preventing any collision with the scenario by using only range readings and the vehicle's relative localization data. Its translation function, therefore, is defined as:

% \begin{equation*}
%     s_t = f(x_t, t_t, m_{t-1}),
% \end{equation*}
% %
% \noindent where $x_t$ is the range findings, $t_t$ is the target's relative information, and $m_{t-1}$ is the vehicle's motion of the last step. These variables describe the current state of $s_t$ of the vehicle. Used in many Deep-RL works for terrestrial mobile robots \cite{tai2017virtual}, \cite{jesus2019deep}, this model helps to obtain the behavior of the agent given its current state.

% \subsubsection{Networks Structure}

The structure of our approaches has a total of 26 dimensions for the state, 20 samples for the distance sensors, the three previous actions and three values related to the target goal, which are the vehicle's relative position to the target, and relative angles to the target in the x-y plane and the z-distance plan. When in the air, the 20 samples come from the LIDAR. We get these samples equally spaced by $13.5\degree$ in the $270\degree$ LIDAR. When underwater, the distance information comes from the Sonar. We also got 20 beams equally spaced among the total of 256, and we took for the highest bin in each beam. This conversion based on the range gives us the distance towards the obstacle or the tank's wall 
\cite{Santos18,Santos19}
.The actions are scaled between $0$ and $0.25$ $m/s$ for the linear velocity, from $-0.25$ $m/s$ to $0.25$ $m/s$ for the altitude velocity and from $-0.25$ to $0.25$ $rad$ for the $\Delta$ yaw.

\subsubsection{Reward Function} % Reescrito por Ricardo

We proposed a binary rewarding function that takes into account a positive reward in case of success or a negative reward in case of failure or in case the episode ($ep$) ends at the 500 steps limit:

\vspace{-5mm}
\begin{equation}
r(s_t, a_t)= 
\begin{cases}
    r_{arrive}           & \text{if } d_t < c_d\\
    r_{collide}          & \text{if } min_x < c_o\ ||\ ep = 500\\
    % c_{r_1}(d_{t-1} - d_t)& \text{if } (d_{t-1} - d_t) \in \mathbb{R}\\
    %> 0\\
    %c_r2               & \text{if } (d_{t-1} - d_t) \leq 0\\
\end{cases}
\end{equation}

The reward $r_{arrive}$ is set to  100, while the negative reward $r_{collide}$ is set to -10. Both $c_d$ and $c_o$ distance were set to $0.5$ meters.

==> whatever/sections/4_experimental_results.tex <==
\section{Experimental Results}
\label{results} % Reescrito por RIcardo

During the training phase, we created a randomly generated goal that the agent should navigate towards. The agents train for a maximum of 500 steps or until they collide with an obstacle or with the tank border. In case of reaching the goal before the limit of episodes, a new random goal was generated. In this case, the total amount of reward could exceed the maximum value of 100. It was used a learning rate of $10^{-3}$, a minibatch of 256 samples and the Adam optimizer for all approaches, including for the compared methods. We limited the number of episodes of 1500 episodes. These respective limits for the episode number ($max\_steps$) are used based on the stagnation of the maximum average reward received.

\subsection{Results} % Reescrito por Ricardo

In this section, the results obtained during our evaluation are shown. An extensive amount of statistics are collected. The task addressed is goal-oriented navigation considering medium transition, where the robot must navigate from a starting point to an endpoint. This task was addressed in a two-fold way in our tests: starting in the air, performing the medium transition and navigating to a target underwater; and the other way around, starting underwater, performing the medium transition and navigating to a target in the air. We collected the statistics for each of our proposed models (DoCRL-D and DoCRL-S) and compared them with the performance of the state-of-the-art deterministic (Det.) and stochastic (Sto.) Deep-RL methods for HUAUVs 
% \cbox{ aqui eu chamaria mesmo de 3DNDRL-D e 3DNDRL-S e citaria o grande 2021, chama "menos atenção" para o fato do grando ser tu mesmo.}
, as well as a behavior-based algorithm \cite{marino2016minimalistic} 
% \cbox{tb nao coloria tanta "atençaõ" para o BBA, chamaria de BBA, behaviour-based algorithm, e explicaria que é baseado no BBA e pronto. POis BBA ja causa uma rejeição pois é meio "toy".}
. This two-fold task was performed for 100 trials and the total of successful trials are recorded. Also, the average time for both underwater ($t\_water$) and aerial ($t\_air$) along navigation with their standard deviations are recorded. 
% However, \textit{we used the models trained in the second environment for the third environment}. We aim to outline one of the main contributions of this work, \textit{i.e.} the robust capacity to generalize of our method across environments, in this case performing in a third, unknown and more complex environment. 

\begin{table}[bp!]
\vspace{-5mm}
\centering
\setlength{\tabcolsep}{0.8pt}
\caption{Mean and standard deviation metrics over 100 navigation trials for all approaches.}
\label{table:mean_std}
\begin{tabular}{c c c c c} 
\toprule
Test & $t_{air}$ (s) & $t_{water}$ (s) & Success \\
\midrule
% 1 & A-W DoCRL-D & $76.28$ $\pm$ $63.20$ & $12.51$ $\pm$ $20.71$ & 94 \\
% 1 & A-W DoCRL-S & $21.79$ $\pm$ $4.57$ & $25.58$ $\pm$ $5.70$ & $100$ \\
% % 1 & A-W 3DNDRL-LD & $13.7$ $\pm$ $1.28$ & $7.02$ $\pm$ $1.14$ & $100$ \\
% % 1 & A-W 3DNDRL-2D & $12.9$ $\pm$ $0.46$ & $5.32$ $\pm$ $0.57$ & $100$ \\
% 1 & A-W Sto. Grando \emph{et al.} \cite{bedin2021deep} & $42.46$ $\pm$ $62.94$ & $13.13$ $\pm$ $15.15$ & $42$ \\
% 1 &\textbf{ A-W Det. Grando \emph{et al.} \cite{bedin2021deep}} & $\textbf{13.84}$ $\pm$ $\textbf{2.11}$ & $\textbf{5.44}$ $\pm$ $\textbf{1.73}$ & $\textbf{100}$ \\
% 1 & A-W BBA & $32.42$ $\pm$ $1.79$ & $21.27$ $\pm$ $0.18$ & $100$ \\
% 1 & W-A DoCRL-D & $24.66$ $\pm$ $10.06$ & $5.0$ $\pm$ $0.71$ & $83$ \\
% 1 & W-A DoCRL-S & $79.73$ $\pm$ $27.91$ & $5.41$ $\pm$ $0.34$ & $100$ \\
% % 1 & W-A 3DNDRL-LD & $13.59$ $\pm$ $1.26$ & $5.15$ $\pm$ $0.79$ & $100$ \\
% % 1 & W-A 3DNDRL-2D & $15.97$ $\pm$ $7.65$ & $5.77$ $\pm$ $1.29$ & $99$ \\
% 1 & W-A Sto. Grando \emph{et al.} \cite{bedin2021deep} & $33.60$ $\pm$ $26.27$ & $6.30$ $\pm$ $2.44$ & $75$ \\
% 1 & \textbf{W-A Det. Grando \emph{et al.} \cite{bedin2021deep}} & $\textbf{15.24}$ $\pm$ $\textbf{2.11}$ & $\textbf{5.41}$ $\pm$ $\textbf{0.43}$ & $\textbf{100}$ \\
% 1 & W-A BBA & $27.44$ $\pm$ $1.68$ & $3.84$ $\pm$ $0.30$ & $100$ \\
\textbf{A-W DoCRL-D} & $\textbf{14.55}$ $\pm$ $\textbf{0.87}$ & $11.19$ $\pm$ $2.86$ & $\textbf{100}$ \\
\textbf{A-W DoCRL-S} & $72.02$ $\pm$ $24.33$ & $\textbf{9.97}$ $\pm$ $\textbf{6.05}$ & $\textbf{70}$ \\
% 2 & A-W 3DNDRL-LD & $23.79$ $\pm$ $12.74$ & $9.67$ $\pm$ $9.49$ & $23$ \\
% 2 & A-W 3DNDRL-2D & $52.41$ $\pm$ $26.24$ & $3.43$ $\pm$ $6.21$ & $2$ \\
A-W Sto. Grando \emph{et al.} \cite{bedin2021deep} & $18.10$ $\pm$ $7.91$ & $1.08$ $\pm$ $2.38$ & $1$ \\
A-W Det. Grando \emph{et al.} \cite{bedin2021deep} & $34.09$ $\pm$ $23.85$ & $13.06$ $\pm$ $12.98$ & $14$ \\
A-W BBA & $34.70$ $\pm$ $30.22$ & $4.87$ $\pm$ $6.16$ & $11$ \\
\textbf{W-A DoCRL-D} & $\textbf{16.67}$ $\pm$ $\textbf{10.44}$ & $\textbf{4.65}$ $\pm$ $\textbf{0.69}$ & $\textbf{42}$ \\
\textbf{W-A DoCRL-S} & $\textbf{8.77}$ $\pm$ $\textbf{7.23}$ & $\textbf{5.98}$ $\pm$ $\textbf{1.90}$ & $\textbf{71}$ \\
% 2 & W-A 3DNDRL-LD & $19.05$ $\pm$ $15.53$ & $7.52$ $\pm$ $4.66$ & $11$ \\
% 2 & W-A 3DNDRL-2D & $24.96$ $\pm$ $29.69$ & $13.44$ $\pm$ $13.20$ & $6$ \\
W-A Sto. Grando \emph{et al.} \cite{bedin2021deep} & $15.33$ $\pm$ $23.75$ & $14.9$ $\pm$ $18.88$ & $12$ \\
W-A Det. Grando \emph{et al.} \cite{bedin2021deep} & $27.58$ $\pm$ $14.77$ & $12.65$ $\pm$ $7.89$ & $13$ \\
W-A BBA & $38.01$ $\pm$ $29.83$ & $3.79$ $\pm$ $0.27$ & $32$ \\

% 3 & \textbf{A-W DoCRL-D} & $61.94$ $\pm$ $45.29$ & $\textbf{8.44}$ $\pm$ $\textbf{9.09}$ & $\textbf{73}$ \\
% 3 & \textbf{A-W DoCRL-S} & $\textbf{14.89}$ $\pm$ $\textbf{1.120}$ & $18.48$ $\pm$ $6.24$ & $\textbf{94}$ \\
% % 3 & A-W 3DNDRL-LD & $23.79$ $\pm$ $12.74$ & $9.67$ $\pm$ $9.49$ & $23$ \\
% % 3 & A-W 3DNDRL-2D & $52.41$ $\pm$ $26.24$ & $3.43$ $\pm$ $6.21$ & $2$ \\
% 3 & A-W Sto. Grando \emph{et al.} \cite{bedin2021deep} & - & - & $0$ \\
% 3 & A-W Det. Grando \emph{et al.} \cite{bedin2021deep} & - & - & $0$ \\
% 3 & A-W BBA & $39.69$ $\pm$ $21.92$ & $11.32$ $\pm$ $7.46$ & $28$ \\
% 3 & \textbf{W-A DoCRL-D} & $\textbf{8.54}$ $\pm$ $\textbf{4.44}$ & $\textbf{4.27}$ $\pm$ $\textbf{0.47}$ & $\textbf{8}$ \\
% 3 & \textbf{W-A DoCRL-S} & $\textbf{15.43}$ $\pm$ $\textbf{13.39}$ & $\textbf{6.60}$ $\pm$ $\textbf{1.75}$ & $\textbf{10}$ \\
% % 3 & W-A 3DNDRL-LD & $19.05$ $\pm$ $15.53$ & $7.52$ $\pm$ $4.66$ & $11$ \\
% % 3 & W-A 3DNDRL-2D & $24.96$ $\pm$ $29.69$ & $13.44$ $\pm$ $13.20$ & $6$ \\
% 3 & W-A Sto. Grando \emph{et al.} \cite{bedin2021deep} & - & - & $0$ \\
% 3 & W-A Det. Grando \emph{et al.} \cite{bedin2021deep} & - & - & $0$ \\
% 3 & W-A BBA & $34.3$ $\pm$ $22.93$ & $6.13$ $\pm$ $17.22$ & $8$ \\
\bottomrule
\end{tabular}
\end{table}

% \begin{figure*}[bp!]
% \vspace{-6mm}
%   \centering
%   \subfloat[DoCRL-D, first env, air-water.\label{fig:cmd_ddpg_1_air_to_water}]{
% 	\begin{minipage}[c][0.65\width]{0.242\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/cmd_td3_stage_1_air_to_water_air3D_tanh_lstm.png}
% 	\end{minipage}}
%  \hfill 	
%   \subfloat[DoCRL-S, first env, air-water.\label{fig:cmd_sac_1_air_to_water}]{
% 	\begin{minipage}[c][0.65\width]{0.242\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/cmd_sac_stage_1_air_to_water_air3D_tanh_lstm.png}
% 	\end{minipage}}
%   \hfill 	
%   \subfloat[DoCRL-D, second env, air-water.\label{fig:cmd_ddpg_2_air_to_water}]{
% 	\begin{minipage}[c][0.65\width]{0.242\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/cmd_td3_stage_2_air_to_water_air3D_tanh_lstm.png}
% 	\end{minipage}}
%   \hfill
%   \subfloat[DoCRL-S, second env, air-water.\label{fig:cmd_sac_2_air_to_water}]{
% 	\begin{minipage}[c][0.65\width]{0.242\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/cmd_sac_stage_2_air_to_water_air3D_tanh_lstm.png}
% 	\end{minipage}}
%   \hfill
%   \vspace{-2mm}
%   \subfloat[DoCRL-D, first env, water-air.\label{fig:cmd_ddpg_1_water_to_air}]{
% 	\begin{minipage}[c][0.65\width]{0.242\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/cmd_td3_stage_1_water_to_air_air3D_tanh_lstm.png}
% 	\end{minipage}}
%  \hfill 	
%   \subfloat[DoCRL-S, first env, water-air.\label{fig:cmd_sac_1_water_to_air}]{
% 	\begin{minipage}[c][0.65\width]{0.242\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/cmd_sac_stage_1_water_to_air_air3D_tanh_lstm.png}
% 	\end{minipage}}
%   \hfill 	
%   \subfloat[DoCRL-D, second env, water-air.\label{fig:cmd_ddpg_2_water_to_air}]{
% 	\begin{minipage}[c][0.65\width]{0.242\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/cmd_td3_stage_2_water_to_air_air3D_tanh_lstm.png}
% 	\end{minipage}}
%   \hfill 	
%   \subfloat[DoCRL-S, second env, water-air.\label{fig:cmd_sac_2_water_to_air}]{
% 	\begin{minipage}[c][0.65\width]{0.242\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/cmd_sac_stage_2_water_to_air_air3D_tanh_lstm.png}
% 	\end{minipage}}
%   \hfill
%   \vspace{-1mm}
%   \caption{Mean and standard deviation of our new proposed agents in each simulated scenario during the 100 navigation trials.}
%   \label{fig:cmd}
% \end{figure*}

We set the initial position for the Air-Water (A-W) trials to (0.0, 0.0, 2.5) in the Gazebo Cartesian coordinates for the three scenarios. The target position was set to (2.0, 3.0, -1.0) at the bottom of the water tank. For the Water-Air (W-A) evaluation, the coordinates were swapped. The same was done for the second and third scenarios, where the coordinates used were (0.0, 0.0, 2.5) and (3.6, -2.4, -1.0). The target was defined in a path with obstacles on the way.
% , while in the third it was a complex configuration simulating risers and inner walls.

% We also collected the reward obtained during the training phase. In the first scenario, we collected the data for 1000 episodes, while the data of 1500 episodes are collected in the second scenario. Overall, Figures \ref{fig:reward_1} and \ref{fig:reward_2} show the rewards' moving average of the previous 300 episodes for the first and second scenarios, respectively. Table \ref{table:mean_std} shows the results obtained for each environment for 100 navigation trials.

% \begin{figure}[tbp!]
% \vspace{-4mm}
%   \subfloat[First environment.\label{fig:reward_1}]{
% 	\begin{minipage}[c][0.72\width]{
% 	   0.485\linewidth}
% 	   \centering
% 	   \includegraphics[width=\linewidth]{img/reward_env1_v3.png}
% 	\end{minipage}}
%  \hfill 	
%   \subfloat[Second environment.\label{fig:reward_2}]{
% 	\begin{minipage}[c][0.72\width]{
% 	   0.485\linewidth}
% 	   \centering
% 	   \includegraphics[width=\linewidth]{img/reward_env2_v3.png}
% 	\end{minipage}}
% \caption{Moving average of the reward over 300 episodes of training.}
% \label{fig:rewards}
% \vspace{-6.5mm}
% \end{figure}





% Specifically, we also performed a complementary comparison in the third scenario. We used the models trained in the second environment to collect the statistics as discussed previously. For a better analysis, we also performed a comparison between models in this third environment. First, we collected the data for DoCRL-D and DoCRL-S models trained only in the second environment for 1500 episodes (Env2), as shown before. Then, we trained these models for 500 more episodes in the third environment (Both). For last, we compared them with DoCRL-D and DoCRL-S trained only in the third environment for 1500 episodes. Table \ref{table:Comparistion_lstm} shows the obtained results.

% \begin{table}[tp!]
% \centering
% \setlength{\tabcolsep}{2.5pt}
% \caption{Mean and standard deviation metrics over 100 navigation trials test in the third simulated environment only, for both DoCRL-D and DoCRL-S models trained only in the second environment (Env2), in both second and third environments (Both), and only in the third environment (Env3).}
% \label{table:Comparistion_lstm}
% \begin{tabular}{c c c c c} 
% \toprule
% Model & $t_{air}$ (s) & $t_{water}$ (s) & Success \\
% \midrule
% \textbf{A-W DoCRL-D (Env2)} & $61.94$ $\pm$ $45.29$ & $\textbf{8.44}$ $\pm$ $\textbf{9.09}$ & $\textbf{73}$ \\
% \textbf{A-W DoCRL-S (Env2)} & $\textbf{14.89}$ $\pm$ $\textbf{1.120}$ & $18.48$ $\pm$ $6.24$ & $\textbf{94}$ \\
% \textbf{A-W DoCRL-D (Both)} & $\textbf{14.14}$ $\pm$ $\textbf{3.77}$ & $\textbf{8.69}$ $\pm$ $\textbf{3.17}$ & $\textbf{99}$ \\
% \textbf{A-W DoCRL-S (Both)} & $16.82$ $\pm$ $2.12$ & $14.92$ $\pm$ $3.60$ & $\textbf{100}$ \\
% A-W DoCRL-D (Env3) & $23.17$ $\pm$ $31.12$ & $32.53$ $\pm$ $60.28$ & $21$ \\
% A-W DoCRL-S (Env3) & $19.98$ $\pm$ $15.99$ & $49.61$ $\pm$ $27.86$ & $87$ \\

% W-A DoCRL-D (Env2) & $8.54$ $\pm$ $4.44$ & $4.27$ $\pm$ $0.47$ & $8$ \\
% W-A DoCRL-S (Env2) & $15.43$ $\pm$ $13.39$ & $6.60$ $\pm$ $1.75$ & $10$ \\
% \textbf{W-A DoCRL-D (Both)} & $\textbf{25.09}$ $\pm$ $\textbf{38.86}$ & $\textbf{4.62}$ $\pm$ $\textbf{0.51}$ & $\textbf{34}$ \\
% \textbf{W-A DoCRL-S (Both)} & $33.41$ $\pm$ $11.82$ & $11.40$ $\pm$ $2.38$ & $\textbf{83}$ \\
% W-A DoCRL-D (Env3) & - & - & $0$ \\
% W-A DoCRL-S (Env3) & $3.73$ $\pm$ $2.97$ & $30.47$ $\pm$ $9.47$ & $1$ \\
% \bottomrule
% \end{tabular}
% \vspace{-4mm}
% \end{table}

% We also performed an analysis of the actions taken by the agents in each scenario for 100 navigation trials. Fig. \ref{fig:cmd} shows the mean of each action value and its standard deviation at each step for these trials. For the last, Fig. \ref{fig:traj_nav} shows a sample of the navigation performed by our new approaches.

\begin{figure*}[tp!]
% \vspace{-10mm}
\centering
%   \subfloat[DoCRL-D behavior in transition air-water. \label{fig:ddpg_1_air_to_water}]{
% 	\begin{minipage}[c][0.73\width]{0.15\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/td3_stage_1_air_to_water_air3D_tanh_lstm.png}
% 	\end{minipage}}
%  \hfill 	
%   \subfloat[DoCRL-S behavior in transition air-water. \label{fig:sac_1_air_to_water}]{
% 	\begin{minipage}[c][0.73\width]{0.15\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/sac_stage_1_air_to_water_air3D_tanh_lstm.png}
% 	\end{minipage}}
%  \hfill	
%  \subfloat[BBA behavior in transition air-water. \label{fig:bug_1_air_to_water}]{
% 	\begin{minipage}[c][0.73\width]{0.15\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/bug_1_air_to_water.png}
% 	\end{minipage}}
%  \hfill
% %  \vspace{-6mm}
%  \subfloat[DoCRL-D behavior in transition water-air. \label{fig:ddpg_1_water_to_air}]{
% 	\begin{minipage}[c][0.73\width]{0.15\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/td3_stage_1_water_to_air_air3D_tanh_lstm.png}
% 	\end{minipage}}
%  \hfill 	
%   \subfloat[DoCRL-S behavior in transition water-air. \label{fig:sac_1_water_to_air}]{
% 	\begin{minipage}[c][0.73\width]{0.15\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/sac_stage_1_water_to_air_air3D_tanh_lstm.png}
% 	\end{minipage}}
%  \hfill	
%  \subfloat[BBA behavior in transition water-air. \label{fig:bug_1_water_to_air}]{
% 	\begin{minipage}[c][0.73\width]{0.15\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{img/bug_1_water_to_air.png}
% 	\end{minipage}}
%  \hfill
% %  \vspace{-6mm}
 \subfloat[DoCRL-D, air-water. \label{fig:ddpg_2_air_to_water}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/td3_stage_2_air_to_water_air3D_tanh_lstm.png}
	\end{minipage}}
 \hfill	
 \subfloat[DoCRL-D, air-water, x-y plane. \label{fig:ddpg_2_air_to_water_2d}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/cmd_td3_stage_2_air_to_water_air3D_tanh_lstm_upper.png}
	\end{minipage}}
 \hfill	
 \subfloat[DoCRL-D, water-air. \label{fig:ddpg_2_water_to_air}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/td3_stage_2_water_to_air_air3D_tanh_lstm.png}
	\end{minipage}}
 \hfill	
 \subfloat[DoCRL-D, water-air, x-y plane. \label{fig:ddpg_2_water_to_air_2d}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/cmd_td3_stage_2_water_to_air_air3D_tanh_lstm_upper.png}
	\end{minipage}}
 \hfill
%  \vspace{-6mm}
 \subfloat[DoCRL-S, air-water. \label{fig:sac_2_air_to_water}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/sac_stage_2_air_to_water_air3D_tanh_lstm.png}
	\end{minipage}}
 \hfill
 \subfloat[DoCRL-S, air-water, x-y plane. \label{fig:sac_2_air_to_water_2d}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/cmd_sac_stage_2_air_to_water_air3D_tanh_lstm_upper.png}
	\end{minipage}}
 \hfill
 \subfloat[DoCRL-S, water-air. \label{fig:sac_2_water_to_air}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/sac_stage_2_water_to_air_air3D_tanh_lstm.png}
	\end{minipage}}
 \hfill
 \subfloat[DoCRL-S, water-air, x-y plane. \label{fig:sac_2_water_to_air_2d}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/cmd_sac_stage_2_water_to_air_air3D_tanh_lstm_upper.png}
	\end{minipage}}
 \hfill
%  \vspace{-3mm}
 \subfloat[BBA, air-water. \label{fig:bug_2_air_to_water}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/bug_2_air_to_water.png}
	\end{minipage}}
 \hfill
 \subfloat[BBA, air-water, x-y plane. \label{fig:bug_2_air_to_water_2d}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/bug_2_air_to_water_upper.png}
	\end{minipage}}
 \hfill
 \subfloat[BBA, water-air. \label{fig:bug_2_water_to_air}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/bug_2_water_to_air.png}
	\end{minipage}}
 \hfill
 \subfloat[BBA, water-air, x-y plane. \label{fig:bug_2_water_to_air_2d}]{
	\begin{minipage}[c][0.73\width]{0.241\textwidth}
	   \centering
	   \includegraphics[width=\textwidth]{img/bug_2_water_to_air_upper.png}
	\end{minipage}}
 \hfill
\caption{Behavior sample of each approach tested in the environment trained. (\cref{fig:ddpg_2_air_to_water,fig:ddpg_2_air_to_water_2d,fig:ddpg_2_water_to_air,fig:ddpg_2_water_to_air_2d,fig:sac_2_air_to_water,fig:sac_2_air_to_water_2d,fig:sac_2_water_to_air,fig:sac_2_water_to_air_2d,fig:bug_2_air_to_water,fig:bug_2_air_to_water_2d,fig:bug_2_water_to_air,fig:bug_2_water_to_air_2d}).}
\label{fig:traj_nav}
\vspace{-6mm}
\end{figure*}


==> whatever/sections/5_discussion.tex <==
\section{Discussion}
\label{discussion}

% REESCREVER, FALAR QUE TD3 E SAC FICARAM MELHOR QUEDDPG E BUG2. FALAR SEMELHANTE AO QUE FOI FEITO NO PAPER DO JINT 

The evaluation shows an overall increase in performance in navigation through the the scenario.  We can see that the DoCRL-D approach achieves a consistent performance of 100 successfully air-to-water navigation trials with also a consistent navigation time ($14.55 \pm 0.87$ and $11.19 \pm 2.86$). In this same scenario, the DoCRL-S approach performed a little worse in air-to-water navigation but outperformed the deterministic approach in water-to-air navigation. 

% In the third scenario, we can see more clearly that a double-critic-based approach with an RNN structure also has a better ability to learn and generalize the environment, including the obstacles and the medium transition. While the state-of-the-art approaches with a MLP structure were not capable to perform the task, our approaches presented once again a consistent performance especially in air-to-water navigation. Our approaches showed an excellent ability to learn the tasks and the environmental difficulties, not only the scenario itself. That was further addressed in our additional evaluation with agents trained in the third environment and both second and third environments. Overall, we can conclude that double critic approaches with recurrent neural networks present a consistent ability to learn through scenarios. Also, our approaches outperformed the BBA algorithm 
% \cbox{BUG2 algorithm - CHamaria de behaviour-based algorithm ou algo assim} 
% in the rate of successful trials and average time in almost all situations.

It is important to mention that these approaches are extensively evaluated in a realistic simulation, including control issues and disturbances such as wind. Thus, the results indicate that our approach may achieve real-world application if the correct data from the sensing and the relative localization are correctly ensured. 
% Finally, it is also possible to analyze that these new RNN-based approaches provided a more consistent average course of actions throughout the environments. 
% We can see in Fig.~\ref{fig:cmd} a decrease in the action's standard deviation when compared with the action's standard deviation of the state-of-the-art~\cite{bedin2021deep}. 

% The extensive validation of our proposed reveals a proper behavior for both agents in both environments. The agents were able to learn environmental difficulties, realize the medium transition, and generalize enough to perform the mapless navigation through air and water. Besides that, our agents also learned to bypass obstacles to arrive at a target and managed to outperform a traditional algorithm. We have validated two powerful approaches, which managed to understand the complex behaviors in realistic simulation and that can be used in the real world if guarantying range findings and relative localization data. 

% Specifically, we can also observe that our deterministic approach performed considerably better than our 3DNDRL-S approach in the first and simpler scenario with just simulated wind and a water tank. However, in the second scenario with simulated drilling risers, we can observe based on the results of Table \ref{table:mean_std} and Figs. \ref{fig:traj_nav_1} and \ref{fig:traj_nav_2} that the better exploration policy of the 3DNDRL-S approach made it have a similar or even better performance than our deterministic algorithm. Finally, it is interesting to notice that, besides the fact that our two approaches have fundamental differences in its implementation, the actions generated by each of them at each step of testing when averaged 100 times are quite similar, manly in the second and more complex scenario. We can observe this robustness and consistency in Fig. \ref{fig:cmd}.



==> whatever/sections/6_conclusion.tex <==
\section{Conclusions}
\label{conclusion}

In this paper, we presented two novels Deep-RL approaches based on RNNs and double critic structures to perform the navigation of a HUAUV. By using physically realistic simulation in several water-tank-based scenarios, we showed that our approaches achieved an overall better capability to perform autonomous navigation, obstacle avoidance and medium transition than other approaches. Disturbances such as wind were successfully assimilated and good generalization through different scenarios was achieved. With our simple and realistic sensing approach that took into account only the range information, we presented overall better performance than the state-of-the-art and a classical behavior-like algorithm. Our work aims to contribute to future studies focusing on rescue missions in robotics, particularly with vehicles like the HUAUV, and extending to environmental rescue tasks in both air and water domains. Furthermore, we are actively conducting research to use our HUAUV model to explore its potential in practical real world applications.


==> whatever/sections/7_acknowledgment.tex <==
%\vspace{-4mm}
\section*{Acknowledgment}

% \anonymize{xx}

%This work was partly founded by the Coordenação de Aperfeiçoamento de Pessoal de Nível Superior (CAPES) and Conselho Nacional de Desenvolvimento Científico e Tecnológico (CNPq). 
The authors would like to thank the VersusAI team. This work was partly supported by the CAPES, CNPq and PRH-ANP.

\vspace{-2mm}

==> whatever/sections/8_references.tex <==
\bibliographystyle{./bibliography/IEEEtran}
\bibliography{./bibliography/IEEEabrv,./bibliography/IEEEexample}

